Exemplar-based Pattern Synthesis with Implicit Periodic Field Network

Synthesis of ergodic, stationary visual patterns is widely applicable in texturing, shape modeling, and digital content creation. The wide applicability of this technique thus requires the pattern synthesis approaches to be scalable, diverse, and authentic. In this paper, we propose an exemplar-based visual pattern synthesis framework that aims to model the inner statistics of visual patterns and generate new, versatile patterns that meet the aforementioned requirements. To this end, we propose an implicit network based on generative adversarial network (GAN) and periodic encoding, thus calling our network the Implicit Periodic Field Network (IPFN). The design of IPFN ensures scalability: the implicit formulation directly maps the input coordinates to features, which enables synthesis of arbitrary size and is computationally efficient for 3D shape synthesis. Learning with a periodic encoding scheme encourages diversity: the network is constrained to model the inner statistics of the exemplar based on spatial latent codes in a periodic field. Coupled with continuously designed GAN training procedures, IPFN is shown to synthesize tileable patterns with smooth transitions and local variations. Last but not least, thanks to both the adversarial training technique and the encoded Fourier features, IPFN learns high-frequency functions that produce authentic, high-quality results. To validate our approach, we present novel experimental results on various applications in 2D texture synthesis and 3D shape synthesis.

==> figures/fig_res_modelnet_ablation.tex <==
\begin{figure}[t]
 \begin{center}
  \centering
  \includegraphics[width=1.0\linewidth]{tsne_cls}
 \end{center}
 \caption{t-SNE embeddings of the equivariant features of 200 airplanes 3D shapes, learnt by different pooling methods. Each datapoint, drawn as circle, is a feature of a single airplane instance defined at rotation group $\soAnc \in \SoAncGroup$. The circles are colored by their associated rotation. The sharp contrast in clustering behaviors are very indicative of how choice of pooling method affects group structures in learned features. }
% \vspace{-10pt}
 \label{fig:pool_tsne}
\end{figure}

==> figures/fig_teaser.tex <==
\begin{figure}[!h]
 \begin{center}
  \centering
  \includegraphics[width=0.8\linewidth]{cvpr22/figs/handdrawn/teaser_vert.png}
 \end{center}
 \caption{ Examples of our target space of synthesis: \textbf{a.} Texture synthesis in infinite domains. \textbf{b.} Synthesis of 3D foam structures. \textbf{c.} Synthesis of seamless 3D textures. Our implicit formulation allows efficient synthesis of patterns that are not limited to 2D texture images. Hence we term our targeted task \textit{pattern synthesis}.}
 
 \label{fig:teaser}
\end{figure}

% \teaser{
% \centering
% \subfloat[Subfigure caption A\label{subfig:fig4a}]{
%     \includegraphics[width=1.0\textwidth]{cvpr22/figs/handdrawn/teaser.png} %standard image inclusion call
% }   ~

% \caption{Teaser pic}
% \label{fig:figure3}
% }

==> figures/sketch.tex <==
\begin{figure}[t]
 \begin{center}
  \centering
 \vspace{-25pt}
  \includegraphics[width=0.9\linewidth]{error_percentile.pdf}
 \end{center}
 \vspace{-20pt}
 \caption{Percentile of errors comparing KPConv~\cite{thomas2019kpconv} and two equivariant models (Ours-N) varied in number of \soThree{} elements.}
 \label{fig:pose}
 \vspace{-10pt}
\end{figure}

==> hackbibstyle.tex <==
\setlength{\topsep}{0ex}
\setlength{\itemsep}{0ex}
\setlength{\partopsep}{0ex}
\setlength{\parsep}{0ex}
\setlength{\parskip}{1ex}
%\footnotesize


==> note.tex <==
\section{Note}
\label{sec:note}


This is note section!
\begin{description}
	\item[Oct. 19, 2019]
	{
		
		\haiwei{I'm good!} %haiwei
		
		\shichen{I'm good!} %shichen
		
		\weikai{I'm good!} %weikai
		
	}
\end{description}


==> sections/implementation.tex <==
\section{Implementation}
\label{sec:imp}

==> sections/method_network.tex <==
\subsection{Implementation Details}
\label{sec:implementation}
%\weikai{put this part to suppl.}
%\paragraph{Sampling Rotation Group.}
%Similar to~\cite{esteves2019equivariant}, we choose to sample the rotation group from an axis-aligned 3D model of regular icosahedron. Each face normal of the icosahedral provides the $\alpha$ and $\beta$ angles. We additionally sample three $\gamma$ angles for each face normal, each separated by 120 degrees. %The rotation is composited from the Euler angles following the xyz standard. The cardinality of the rotation set is thus $20 \times 3=60$. Thanks to the icosahedral symmetry, the sampled set forms a rotation group $\SoAncGroup$ with closure, identity and inverse elements. To enable limited support filters, we further choose a 12-element subgroup to transform $\SoAncGroup$ to its \soThree{} neighbors. 
The core element of our network is the \convNameShort{} block as shown in Fig.~\ref{fig:conv}(d).
%that is analogous to the regular convolutional block. 
It consists of one \convNameInter{} and one \convNameIntra{} operator, with a batch normalization and a leaky ReLU activation inserted in between and after. 
%The convolution block adds skip connection, leaky ReLu activation and batch normalization to the convolution operation. 
%While it is suitable for any convolutional architecture, we design a network \haiwei{name?} following empirical evidence on point cloud architecture. 
We employ a 5-layer hierarchical convolutional network.
Each layer contains two \convNameShort{} blocks, with the first one being strided by a factor of $2$.
The network outputs spatially pooled features that are equivariant to the rotation group \SoAncGroup. It can be then pooled into an invariant feature through a \poolingNameShort{} layer. For the classification network, the feature is fed into a fully connected layer and a \textit{softmax} layer. For the task of metric learning, the feature is processed with an L2 normalization. We provide detailed network parameters and downsampling strategy in the supplemental materials.

%
%\textbf{Downsampling.} Spatial downsampling is performed by strided \ConvNameInter{}. 
%% ($\SphFeat_i \in \mathbb{R}^{\pointNum_i \times \soAncNum \times \soFeatDim_{in}} \rightarrow \SphFeat_{i+1} \in \mathbb{R}^{\pointNum_{i+1} \times \soAncNum \times \soFeatDim_{out}   }$).  
%In particular, the hierarchical sampling and grouping operations in spatial dimension are applied before the strided convolution.
%%Striding point convolution amounts to the hierarchical sampling and grouping of a subset of centers in the spatial dimension prior to the strided convolution. 
%%A low-pass filter is also applied spatially to the grouped features for better robustness to small transformations~\cite{azulay2018deep}.  
%Grouping radius and $\sigma$ (in Equation~\ref{equ:correlation}) are adjusted to increase the receptive field of filters in the subsequent convolutions. To address the resampling issue in point cloud grouping, where the number of points in a neighborhood is less than the desired amount, we attempted both repetitive sampling and the use of shadow points. 
%Though empirical results do not indicate major performance between these two approaches, we choose shadow sampling in our implementation. 
%%We did not find major performance difference between these two approaches and have opted for shadow point sampling. 
%We do not perform downsampling in the \soThree{} dimension due to the difficulties in maintaining rotational equivariance and group properties. 
%
%\weikai{move this to supplemental material}
%\paragraph{Network parameters.} We select a kernel size of 30 with kernel points spread evenly inside a ball $\mathcal{B}_r^3$. The radius $r$ of grouping operator is set as $r^2 = d\sigma$ where $d$ is a parameter related to density of the data. The kernel radius $r_k$ is set as $r_k = 0.7r$. For all experiments, the input are spatial coordinates of point cloud, uniformly subsampled to an input size of $1024 \times 3$. 

%<<<<<<< HEAD
%\paragraph{Network architecture}
%	The core of our network architecture is the \ConvNameFull{} block that is analogous to the regular convolutional block. The convolution block adds skip connection, leaky ReLU activation and batch normalization to the convolution operation. While it is suitable for any convolutional architecture, we design a network \haiwei{name?} following empirical evidence on point cloud architecture. The network is a N-layer fully convolutional network (N=5 for classification, N=4 for matching). Each layer contains two \ConvNameFull blocks, with the first one being strided. The last layer contains two unary convolution layers. After the last layer, a global average pooling is first performed in the spatial dimension. The resulted group equivariant feature is then pooled into an invariant feature through \poolingName. For the classification network, the feature is then processed by fully connected and softmax layers. For the metric learning network, the feature is processed with a L2 normalization. 
%=======




==> sections/method_overview.tex <==
%\subsection{Overview}
%\label{sec:overview}



% Point and Rotation Group Representations
%<<<<<<< HEAD
%	We denote a rotation group $\SoAncGroup$, where $\soAnc \in \SoAncGroup$ is associated with a rotation $\soRot \in \soThree$. $\SoAncGroup$ is thus a discrete subset of the continuous group \soThree. The order of $\SoAncGroup$ ($\vert \SoAncGroup \vert$) is denoted \soAncNum. We denote a 3D point as $\point$ from a set of points $\Point \in \mathbb{R}^{\pointNum \times 3}$. The equivariant representation of point feature is a function $\SoFeat(\point,\soAnc): \mathbb{R}^3 \times \SoAncGroup \rightarrow \mathbb{R}^D$. Different from the feature space $\SoFeat(\point): \mathbb{R}^3 \rightarrow \mathbb{R}^D$ used in many shift-invariant point set convolution, $\SoFeat$ contains dimensionally lifted features that are also defined on elements of the rotation group $\SoAncGroup$. For intuitiveness, we call $\SoFeat(\point,\soAnc)$ the feature of a point $\point$ at \textbf{anchor} $\soAnc$. 
%=======
\paragraph{Overview.}

%\haiwei{
In this section, we first start with the preliminaries of \seThree{} convolutions. We will then provide the detailed mathematical formulation of our approach: (1) the \seThree{} separable convolution; and (2) attention mechanism for the equivariant features. 
%}
The Lie group \seThree{} is the group of rigid body transformations in three-dimensions: 
\begin{align*}
\seThree = \{ A \vert A = 
\begin{bmatrix}
	R & t \\
	0 & 1
\end{bmatrix}, R \in  \soThree, t \in  \mathbb{R}^{3}\}. 
\end{align*}

\noindent \seThree{} is homeomorphic to $\mathbb{R}^{3} \times \soThree$. Therefore, a function that is equivariant to \seThree{} must be equivariant to both 3D translation $ t \in \mathbb{R}^{3}$ and 3D rotation $ g \in \soThree $. Given a spatial point $\point$ and a rotation $\soAnc$, let us first define the continuous feature representation in \seThree{} as a function $\SoFeat(\pointi,\soAncj): \mathbb{R}^3 \times \soThree \rightarrow \mathbb{R}^D$. Equivariance to \seThree{} is expressed as satisfying $ \forall A \in \seThree,
  A(\SphFeat \ast \kernelFunc)(\point, \soAnc) = (A\SphFeat \ast \kernelFunc)(\point, \soAnc) 
$. The \seThree{} equivariant continuous convolutional operator can be defined as 
\vspace{-2mm}
\begin{multline}
  (\SoFeat \ast \kernelFunc)(\point, \soAnc) \\ =
  \int_{\pointi \in \mathbb{R}^{3}} \int_{\soAncj \in \soThree} \SoFeat(\pointi, \soAncj) \kernelFunc(\soAnc^{-1}(\point - \pointi), \soAncj^{-1}\soAnc)
  \label{equ:6d_conv_continuous},
\end{multline}

% \begin{align}
%     (\SoFeat \ast \kernelFuncInter)(\point, \soAnc) &= \int_{\pointi^\prime \in \mathbb{R}^{3}} \SoFeat(\point - \pointi^\prime, \soAnc) \kernelFuncInter(\soAnc \pointi^\prime, \mathrm{I})
%     \label{equ:separate_inter} \\
%     (\SoFeat \ast \kernelFuncIntra)(\point, \soAnc) &= \int_{\soAncj \in \soThree} \SoFeat(\point, \soAncj^{-1}\soAnc) \kernelFuncIntra(\mathbf{0}, \soAncj)
%   \label{equ:separate_intra}
% \end{align}

\noindent where $\kernelFunc$ is a kernel $\kernelFunc(\point,\soAnc): \mathbb{R}^3 \times \soThree \rightarrow \mathbb{R}^D$. The convolution is computed by translating and rotating the kernel and then computing a dot product with the input function $\SoFeat$. 
%\shichen{Given $D_{out}$ kernels, the convolution produces feature vectors of dimension $D_{out}$ in the domain of \seThree{}.} 
We prove that this convolution is equivariant to \seThree{} in the supplementals.

\vspace{-4mm}
\paragraph{Discretization.} To discretize Eq.~\ref{equ:6d_conv_continuous}, we starts with discretizing the \seThree{} space into a composition of a finite set of 3D spatial point $\Point: \{ \point \vert \point \in  \mathbb{R}^{3} \}$ and a finite rotation group $\SoAncGroup \subset \soThree$.  
 This leads to a discrete \seThree{} feature mapping function $\SoFeat(\pointi,\soAncj): \Point \times \SoAncGroup \rightarrow \mathbb{R}^D$. The discrete convolutional operator in \seThree{} is therefore:

\begin{equation}
  (\SoFeat \ast \kernelFunc)(\point, \soAnc) = \sum_{\pointi \in \Point} \sum_{\soAncj \in \SoAncGroup} \SoFeat(\pointi, \soAncj) \kernelFunc(\soAnc^{-1} (\point - \pointi), \soAncj^{-1}\soAnc).
  \label{equ:6d_conv}
\end{equation}

\noindent We note that such discretization serves as a good approximation of the continuous formulation in Eq.~\ref{equ:6d_conv_continuous}, where the approximation error can be further mitigated by the rotation augmentation~\cite{azulay2018deep}. If we interpret $\Point$ as a set of 3D displacements, this leads to an equivalent definition:
\begin{equation}
\begin{split}
  (\SoFeat \ast \kernelFunc)(\point, \soAnc) &= \sum_{\pointi \in \Point} \sum_{\soAncj \in \SoAncGroup} \SoFeat(\soAnc^{-1}(\point - \pointi), \soAncj^{-1}\soAnc) \kernelFunc(\pointi, \soAncj) \\
  &=  \sum_{\pointi^\prime \in \Point_{\soAnc}} \sum_{\soAncj \in \SoAncGroup} \SoFeat(\point - \pointi^\prime, \soAncj^{-1}\soAnc) \kernelFunc(\soAnc\pointi^\prime, \soAncj).
  \end{split}
  \label{equ:6d_conv_alt}
\end{equation}

\vspace{-1mm}
Without loss of generality, we assume the coordinate is expressed in the local frame of $\point$ and therefore $g^{-1}x = x$. In the second row of Eq.~\ref{equ:6d_conv_alt}, the summation over the set $\Point$ becomes a summation over a rotated set $\Point_\soAnc: \{ \soAnc^{-1}\point \vert \point \in \Point \}$. When written this way, we can see that the kernel is parameterized by a set of translation offsets and rotation offsets under the reference frame given by $\soAnc$.  We call the discrete set $\Point \times \SoAncGroup$ the domain of the kernel with a kernel size of $\vert \Point \vert \times \vert \SoAncGroup \vert$.
%It is worth noting that the discretization limits the above convolutional operator to be only equivariant to the rotation group $\SoAncGroup$. Much like the case with discrete shift-equivariant operator \cite{azulay2018deep}, there is no discrete operator that can be equivariant to the continuous $\soThree$ space. However, equivariance error of a neural network can often be mitigated by techniques such as rotation augmentation.
\vspace{-3mm}
\paragraph{\seThree{} Separable Convolution.}  A key issue with Eq.~\ref{equ:6d_conv_alt} is that the convolution is computed over a 6-dimensional space -- a naive implementation would be computational prohibitive. Inspired by the core idea of separable convolution~\cite{chollet2017xception}, we observe that the kernel $\kernelFunc$ with a kernel size $\vert \Point \vert \times \vert \SoAncGroup \vert$ can be separated into two smaller kernels, denoting $\kernelFuncInter$ with a kernel size of $\vert \Point \vert \times 1 $ and $\kernelFuncIntra$ with a kernel size of $1 \times \vert \SoAncGroup \vert$. This divides the domain of the kernel to two smaller domains: $\Point \times \{\mathrm{I}\}$ for $\kernelFuncInter$, and $\{\mathbf{0}\} \times G$ for $\kernelFuncIntra$, where $\mathrm{I}$ is the identity matrix, and $\mathbf{0}$ is a zero displacement vector. From here, we are ready to separate Eq.~\ref{equ:6d_conv_alt} into two convolutions:
\vspace{-2mm}
\begin{align}
    (\SoFeat \ast \kernelFuncInter)(\point, \soAnc) &= \sum_{\pointi^\prime \in \Point_{\soAnc}} \SoFeat(\point - \pointi^\prime, \soAnc) \kernelFuncInter(\soAnc \pointi^\prime, \mathrm{I})
    \label{equ:separate_inter} \\
    (\SoFeat \ast \kernelFuncIntra)(\point, \soAnc) &= \sum_{\soAncj \in \SoAncGroup} \SoFeat(\point, \soAncj^{-1}\soAnc) \kernelFuncIntra(\mathbf{0}, \soAncj)
  \label{equ:separate_intra}
\end{align}

\vspace{-3mm}
 We can see that $\kernelFuncInter$ is a kernel only varied by translation in the reference frame of $\soAnc$, and $\kernelFuncIntra$ is a kernel only varied by the rotation $\soAncj$. In the following text, we simplify them to $\kernelFuncInter(\soAnc \pointi^\prime)$ and $\kernelFuncIntra(\soAncj)$. The division here matches with the observation that the space \seThree{} can be factorized into two spaces $\mathbb{R}^{3}$ and \soThree{}. 
 Sequentially applying the two convolutions in Eq.~(\ref{equ:separate_inter}-\ref{equ:separate_intra}) approximates the 6D convolution in Eq.~\ref{equ:6d_conv_alt} (Fig.~\ref{fig:conv}(d)) while maintaining equivariance to \seThree{} (proofs provided in the supplementary materials). The working principle here is similar to that of the Inception module~\cite{szegedy2015going} and its follow-up works~\cite{chollet2017xception}, which have shown the promising property of separable convolutions in improving the network performance with reduced cost. We name the two consecutive convolutions as \textit{\convNameInter{}} and \textit{\convNameIntra{}}, respectively, as shown in Fig.~\ref{fig:conv}. We refer the combined convolutions as \textit{\convNameFull{} (\convNameShort{})}.
 Formally, the original 6D convolution is approximated by: $\SoFeat \ast \kernelFunc \approx (\SoFeat \ast \kernelFuncInter) \ast \kernelFuncIntra$.

%
%
%%impractical due to its high computational complexity. 
%However, we observe that the 6D space consists of two relatively independent subspaces.
%To reduce the computational cost, we propose to break down the \seThree{} convolution into two separable convolutions operating in the translational ($\mathbb{R}^{3}$) and rotational (\soThree{}) spaces, respectively.
%Hence, a sequential block of a point convolution defined on $\mathbb{R}^{3}$ followed by a group convolution defined on \soThree{} operating on \seThree{} tensors (Figure~\ref{fig:conv}(d)) could approximate the 6D convolution while maintaining equivariance to the \seThree{} space. 
%The working principle here is similar to that of the Inception module~\cite{szegedy2015going} and its follow-up works~\cite{chollet2017xception}, which have shown the promising property of separable convolutions in improving the network performance with reduced cost.
%
%%\weikai{It is a bit difficult for me to understand the following context. We should explain 1) the insight why the original discretization can be separated in such way; 2) how to obtain the original discretization from the two separable convolutions? 3) why our method is advantageous over the spectral approach?}
%We name the two consecutive convolutions as \textit{\convNameInter{}} and \textit{\convNameIntra{}}, respectively, as shown in Fig.~\ref{fig:conv}. In particular, we divide the kernel function $\kernelFunc(\point, \soAnc)$ into $\kernelFuncInter(\point\ \vert\ \soAnc)$ and $\kernelFuncIntra(\soAnc)$. 
%Formally, the original 6D convolution is approximated by:
%\begin{equation}
%	\SoFeat \ast \kernelFunc \approx (\SoFeat \ast \kernelFuncInter) \ast \kernelFuncIntra.
%\end{equation}
%\vspace{-5mm}
%
%
%\noindent By localizing the operator,  the separable convolutions are:
%
%\begin{align}
%  \left\{
%  \begin{array}{l}
%    (\SoFeat \ast \kernelFuncInter)(\point, \soAnc) = \sum_{\pointi \in \mathcal{N}_\point} \SoFeat(\pointi, \soAnc) \kernelFuncInter(\point - \pointi\ \vert\ \soAnc) \\
%    (\SoFeat \ast \kernelFuncIntra)(\point, \soAnc) = \sum_{\soAncj \in \mathcal{N}_\soAnc} \SoFeat(\point, \soAncj) \kernelFuncIntra(\soAncj^{-1}\soAnc).
%  \end{array}
%  \right.
%\end{align}
%\vspace{-10pt}
%
%We refer the combined convolutions as \textit{\convNameFull{} (\convNameShort{})}.
% Previous works have proposed spectral methods(cite some) and non-spectral methods (cite some) to discretize the convolution operation in \soThree{}. We note that both approaches must start with a discretization of the representation itself. In this work, we choose to incorporate the discrete group convolution on a finite rotation group . Furthermore, to discretize translation, we define $\mathcal{N}_\point$ to be a finite neighborhood around a spatial point $\point \in  \mathbb{R}^{3}$.
%
%The discretization in $\soThree$ limits the above convolutional operator to be only equivariant to the rotation group $\SoAncGroup$. Although there is no discrete operator that can be equivariant to the continuous $\soThree$ space, the equivariance error of a neural network can often be mitigated by rotation augmentation of the data. 
%
%A practical way to define discrete subgroup of \soThree{} is to compute from the faces of Platonic solids (e.g. Tetrahedral, Icosahedral) thanks to their rotational symmetry. This approach is proposed by (cite some) and has been adopted by several group convolutional network (cite some). 
%
%
%In this paper, we use a discrete rotation representation, which is also known as a rotation group $\SoAncGroup$, where each element $\soAncj \in \SoAncGroup$ is associated with a rotation $\soRotj \in \soThree$. 
%Let $\soAncNum$ be the cardinality of the group $\soAncNum = \vert \SoAncGroup \vert$. 
%We denote $\pointi$ as a 3D point belonging to the set $\Point \in \mathbb{R}^{\pointNum \times 3}$. 
%The equivariant representation of point and group feature is a function $\SoFeat(\pointi,\soAncj): \mathbb{R}^3 \times \SoAncGroup \rightarrow \mathbb{R}^D$. 
%Different from the feature space $\mathbb{R}^3 \rightarrow \mathbb{R}^D$ used in many shift-invariant point set convolution, $\SoFeat$ contains dimensionally lifted features that are also defined on the elements of the rotation group $\SoAncGroup$. 
%%\shichen{For intuitiveness, we call $\SoFeat(\pointi,\soAncj)$ the feature of a point $\pointi$ at anchor $\soAncj$.}
%% How separable convolution works
%Let us define the discrete convolutional operator in \seThree{} space as
%\begin{equation}
%  (\SoFeat \ast \kernelFunc)(\point, \soAnc) = \sum_{\pointi \in \mathcal{N}_\point} \sum_{\soAncj \in \mathcal{N}_\soAnc} \SoFeat(\pointi, \soAncj) \kernelFunc(\point - \pointi, \soAncj^{-1}\soAnc),
%  \label{equ:6d_conv}
%\end{equation}
%\noindent where $\kernelFunc$ is a kernel function defined in the 6D space.
%Unfortunately, the naive implementation of such convolution is impractical due to its high computational complexity.
%However, \seThree{} space can be divided into two subspace, namely $\mathbb{R}^3$ and $\soThree$.
%Inspired by the core idea of separable convolution~\cite{chollet2017xception}, we propose to reduce the 6D complexity to 3D by factorizing the \seThree{} convolution into the spatial and  rotational subspaces. 
%We denote them as \textit{\convNameInter{}} and \textit{\convNameIntra{}}, respectively, as shown in Fig.~\ref{fig:conv}.
%In particular, we divide $\kernelFunc(\point, \soAnc)$ into $\kernelFuncInter(\point\ \vert\ \soAnc)$ and $\kernelFuncIntra(\soAnc)$. The convolution thus is given by
%
%\begin{align}
%  \left\{
%  \begin{array}{l}
%    (\SoFeat \ast \kernelFuncInter)(\point, \soAnc) = \sum_{\pointi \in \mathcal{N}_\point} \SoFeat(\pointi, \soAnc) \kernelFuncInter(\point - \pointi\ \vert\ \soAnc) \\
%    (\SoFeat \ast \kernelFuncIntra)(\point, \soAnc) = \sum_{\soAncj \in \mathcal{N}_\soAnc} \SoFeat(\point, \soAncj) \kernelFuncIntra(\soAncj^{-1}\soAnc).
%  \end{array}
%  \right.
%\end{align}
%
%We name these two convolutions as \textit{\convNameFull{} (\convNameShort{})}.
%%while each convolution is defined in a dimensionality of 3.
%% Overall pipeline from input to output
An \seThree{} equivariant convolutional network can be realized by consecutive blocks of \convNameShort{}. 
The network consumes the input $\Point$ and produces an \textit{\seThree{} equivariant} feature for the point set. 
Since \convNameShort{} only takes functions defined on \seThree{} as input, for each point in the input point set, we set $\SoFeat(\point, \soAnc)=1$ for each $\soAnc \in G$. 
%Since the previously defined convolutions accept inputs in the domain $\Point \times \SoAncGroup$ , we propose an extension operator $\mathcal{E}_\point : \mathbb{R}^{3} \rightarrow \mathbb{R}^{3} \times \soThree$. The form of the extension operator depends on the input point feature $F_\Point: \mathbb{R}^{3} \rightarrow \mathbb{R}^{D}$. When the spatial coordinate is used as point feature, $F(\point) = \point$, then $\mathcal{E}_\Point(\point, \soAnc) = g^{-1}\point$.  When $F(\point) = 1$ denoting an occupied space, $\mathcal{E}_\Point(\point, \soAnc) = 1$. 
In the following sections, we discuss in details the form of kernel and how it can be localized for each convolution module.

%
% Specifically, $\Point$ is first lifted to the feature space $\mathbb{R}^{\pointNum \times \soAncNum \times 1}$ 
%\weikai{What is $N$ and $M$, $N_x$ and $N_g$?}%weikai
% and passed through a sequence of \convNameShort{} blocks. 
%The equivariant features at the output layer may be fused into an invariant feature by a \poolingName{} layer (see Section \ref{sec:att}). 
%%The following sections provide detailed formulation of the separated convolution layers.
%The separation of point convolution from \soThree{} convolution enables an intuitive way to extend any formulation of translation-equivariant point convolution into a \seThree{} equivariant convolution. 
%In the following section, we will provide representative examples of extended point convolution operators. 
%We do emphasize the importance of translation-equivariant operator, because it is the key to spatially localize filters and therefore to support a hierarchical convolutional structure. 
%Such framework has seen great success in recent years.

%
%The benefits of such separation are twofold: 1) It drastically decrease computational overhead needed for \seThree{} equivariance (see the following complexity analysis); and 2) the separable framework is non-spectral, thus easy to implement, easily band-limited, and can easily incorporate any shift-equivariant point convolution method. 
%
%\paragraph{Complexity analysis.} As illustrated in Fig.~\ref{fig:conv}, by combining the two equivariance-preserving convolutions, we can achieve similar effect with Equation~\ref{equ:6d_conv} at a much lower computational cost. In particular, we denote $K_p$ and $K_g$ as the number of kernels in the point and group convolution; $C_{i}$ and $C_{o}$ the number of input and output channels. The naive 6D convolution requires a computational complexity of $O(K_pK_gC_{i}C_{o})$. In contrast, the complexity of our approach is reduced to $O(K_pC_{i}+K_gC_{o})$, which could achieve orders-lower complexity compared to the naive solution especially with large $K_p$ and $K_g$.

%For instance, we denote $N$ as the kernel size for parameterizing the convolution in the two subspace $\mathbb{R}^3$ and $\soThree$. The naive 6D convolution requires $N^2$ kernels, which is 10 times the parameters and multiplications needed by our proposed separable convolutions.
%a kernel size of 20 is used to parameterize convolution in the two subspace . A straightforward 6D convolution would require a 20x20 kernel, which results in 10 times the parameters and multiplications needed by two separated convolutions.

%
%% How separable convolution works
%	The \convNameFull{} defined on $\mathbb{R}^3 \times \soThree$ is factorized into a \convNameInter{} followed by a \convNameIntra{}, where \convNameInter{} applies filter on translation correlations in $\mathbb{R}^3$ while \convNameIntra{} applies filter on rotation correlations in $\soThree$. 

==> sections/method_prelim.tex <==
\subsection{Preliminaries}
\label{sec:prelim}

\paragraph{Representation}

A unit 2-sphere $\sphere$ is defined as the set of points $\{(x,y,z)|x^2+y^2+z^2=1\}$ in $\mathbb{R}^3$. 

In this paper, we consider a convex conic region emanating from the origin of a 2-sphere to be a convex spherical sector parameterized by its cone angle $\coneAngle$ (or aperture) and its radius $\coneR$. Additionally, each conic region considered in this paper is given a viewing direction $\coneDirec \in \sphere$ as its axis. The set of points in the conic region is therefore ...


A point convolution can be modeled by the convolution of point features from $\SphFeat \in \mathbb{R}^{\sphFeatNum \times \sphFeatDim}$ and a kernel function $\kernelFunc$ on points $\point_i$ from a point set $\Point \in \mathbb{R}^{\sphFeatNum \times 3}$ in 3D:

\begin{equation} \label{pcconv}
  (\convFunc)(\point) = \sum_{\point_i \in \neighbor_\point} f(\point_i) \kernelFunc(\point_i - \point)
\end{equation} 


Spherical feature $\SphFeat : \sphere \rightarrow \mathbb{R}^\sphFeatDim$. \shichen{don't understand} \haiwei{maybe rename to spherical feature or spherical signal}

Spherical point: given a point set $\Point \in \mathbb{R} ^{\sphFeatNum \times 3}$, spherical points $\{\sphpoint_i (\point_i, \sphFeat_i)\}$ are formed by equipping each point $\point_i \in \Point$ with a spherical feature $\sphFeat_i \in \SphFeat$

\paragraph{Group Equivariance in CNNs} 

\haiwei{

A function $f$ is said to be equivarient to a group $\Group$ if $f(\group(x)) = (L_\group f)(x)$ for all transformations $\group \in \Group$,  where $L_{\group}$ is defined as the group operator that acts on the function $f$. 

The group convolution $$(\groupConvFunc{\group})(\point) = \int_{\group \in \Group} (L_\group f) \kernelFunc(\group^{-1}(\point))d\group$$ is equivariant to $\group$ given integrable functions $f$, $\group$ defined on $\Group$.  The translation group $\group = \mathbb{R}^3$ and the rotation group $\group = SO(3)$ are of special interests to the study of 3D shape analysis. Point convolution in 3D of the form \ref{pcconv}, naturally extending from the familiar discrete convolution, is translation-invariant (given that $h(g(x)) = (L_g h)(x)$). We thus focus our attention on the cases when $\group = SO(3)$ and $\group = SE(3)$.

}

\paragraph{Spherical Convolution}  

The spherical convolution defined in \cite{healy2003ffts} is given by: 

\begin{equation} \label{cont_sph_conv}
	 (\convFunc)(\point) = \int_{SO(3)} \sphFeat(\rotation \northPole)\kernelFunc(\rotation^{-1}\point)d\rotation
\end{equation}

where $\northPole$ is a canonical direction (north pole). Varied from the $\sphere$ correlation defined in \cite{cohen2018spherical}, this formulation allows the output of the convolution to be defined on $\sphere$. An important characteristics in \ref{cont_sph_conv} is that rotation of the canonical north pole $\northPole$ is invariant to Z-axis, therefore imposing $\kernelFunc$ to be circularly symmetric. Specifically, in the spectral domain, the convolution of $\sphFeat$ with the symmetric kernel $\kernelFunc$ is given by a weighted multiplication with Zonal Harmonic coefficients:  \((\convFunc)^m_l = \sqrt{\frac{4\pi}{2l+1}} h^0_lf^m_l\).



==> sections/result_quant.tex <==
\subsection{Quantitative Evaluation}
\label{sec:quant}


==> tables/tab_3dm_ablation.tex <==
\begin{table}[]
%\small
%\addtolength{\tabcolsep}{4pt}
\caption{Average recalls under different alignment settings
} 
\centering
\begin{tabular}{c|c}
%\hline
%Methods &  Mean pool & Max pool & Unsup. atten. & Point conv & Full    \\ \hline
%Accuracy & ? & 87.4 & ? & ? & \textbf{88.3}\\ \hline
%\end{tabular}
\hline
setting &  average recall (\%)   \\ \hline
standard & \textbf{96.6}\\ 
dense & 96.5 \\ 
rotated & - \\ 
aligned & - \\ 
\end{tabular}


\label{tab:3dm_abl}
%\vspace{-7 pt}
\end{table}

==> tables/tab_3dmatch.tex <==


\begin{table*}[h]
\small
\addtolength{\tabcolsep}{1.5pt}
\centering
\begin{tabular}{l|cccccc|cc|c}
\hline
        & SHOT\cite{tombari2010unique} & 3DMatch\cite{zeng20163dmatch} & CGF\cite{khoury2017learning}  & PPFNet\cite{deng2018ppfnet} & PPFF\cite{deng2018ppf} & 3DSNet\cite{gojcic2019perfect} & Li\cite{li2020end} & Li\cite{li2020end}$^\flat$ &   Ours \\ \hline
Kitchen & 74.3 & 58.3    & 60.3 & 89.7   & 78.7        & 97.5    & 92.1 & \textcolor{black}{\textbf{99.4}} & 99.0 \\  %&       \textbf{96.9}
Home 1  & 80.1 & 72.4    & 71.1 & 55.8   & 76.3        & 96.2            & 91.0 & \textcolor{black}{98.7} & \textbf{99.4} \\  %&      \textbf{93.0}
Home 2  & 70.7 & 61.5    & 56.7 & 59.1   & 61.5        & 93.2            & 85.6 & \textcolor{black}{94.7} & \textbf{96.2}\\  %&      83.2
Hotel 1 & 77.4 & 54.9    & 57.1 & 58.0   & 68.1        & 97.4            & 95.1 & \textcolor{black}{\textbf{99.6}} & \textbf{99.6}\\  %&      \textbf{94.7}
Hotel 2 & 72.1 & 48.1    & 53.8 & 57.7   & 71.2        & 92.8            & 91.3 & \textcolor{black}{\textbf{100.0}} & 97.1\\  %&   \textbf{88.5}
Hotel 3 & 85.2 & 61.1    & 83.3 & 61.1   & 94.4        & 98.2             & 96.3 & \textcolor{black}{\textbf{100.0}} & \textbf{100.0} \\ %&   95.6
Study   & 64.0 & 51.7    & 37.7 & 53.4   & 62.0        & 95.0             & 91.8 & \textcolor{black}{95.5} & \textbf{96.2} \\ %&   78.4
MIT Lab & 62.3 & 50.7    & 45.5 & 63.6   & 62.3        & \textbf{94.1}             & 84.4 & \textcolor{black}{92.2} & 93.5\\ \hline %&      77.3
Average & 73.3 & 57.3    & 58.2 & 62.3   & 71.8        & 95.6             & 91.0 & \textcolor{black}{97.5} & \textbf{97.6} \\ \hline %&     \textbf{88.5}
\end{tabular}
\caption{Comparisons of average recall of keypoint correspondences on 3DMatch. 
Li~\cite{li2020end}$^\flat$ denotes results tested with point normal information provided by the authors. All other results are tested on the official 3DMatch evaluation set without point normals.
	%Ours (mp) and ours(att.) denote our approach using max and attentive pooling respectively.
	%The feature dimension of 3DSmoothNet and ours is 32-dim. 
}

\vspace{-5mm}
\label{tab:3dmatch}
\end{table*}

==> tables/tab_modelnet.tex <==
%\begin{table}[]
%\begin{tabular}{l|llll|llll}
%\hline
%& \multicolumn{4}{c}{Color image}    & \multicolumn{4}{|c}{Point cloud}              \\ \hline
%& MVCNN-80~\cite{} & RotationNet & Spherical CNN & CGF  & PPFNet & PPF-FoldNet & 3DSmoothNet(32) & ours \\ \hline
%Kitchen & 43.1 & 74.3 & 58.3    & 60.3 & 89.7   & 78.7        & 97.0            &      \\
%Home1   & 66.7 & 80.1 & 72.4    & 71.1 & 55.8   & 76.3        & 95.5            &      \\ \hline
%\end{tabular}
%\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small
\centering
\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{l|l|c|c}
\hline
\multicolumn{1}{c|}{Representation} & Methods & \multicolumn{1}{l|}{Acc (\%)} & \makecell{Retrieval \\ (mAP)} \\ \hline
\multirow{2}{*}{3D Surface}{\begin{tabular}[c]{@{}c@{}}  \end{tabular}} 
 % & MVCNN-80 & 86.0 & 99M \\
 & RotationNet~\cite{kanezaki2018rotationnet} & 80.0 & 74.2 \\
 & Sph. CNN~\cite{esteves2018learning} & 86.9 & - \\ 
 % & Multiview CNN~\cite{esteves2019equivariant} & \textbf{91.1} & - \\
 \hline
\multirow{6}{*}{Point cloud} 
 & QENet~\cite{zhao2019quaternion} & 74.4 & - \\
 & PointNet~\cite{qi2017pointnet} & 83.6 & - \\
 & PointNet++~\cite{qi2017pointnet++} & 85.0 & 70.3 \\
 & DGCNN~\cite{qi2017pointnet} & 81.1 & - \\
 & PointCNN~\cite{qi2017pointnet++} & 84.5 & - \\ % Li, Y, et. al. PointCNN: Convolution on X-transformed Points\\
 & KPConv~\cite{thomas2019kpconv} & 86.7 & 77.5 \\
 & Ours & \textbf{88.3} & \textbf{79.7} \\ \hline
\end{tabular}
\caption{Results on shape classification and retrieval on randomly rotated objects of ModelNet40. 
	%We compare our testing accuracy with previous methods on rotated ModelNet40 dataset, where each training and testing data is perturbed with a random rotation
	%color in \textcolor{blue}{blue} denotes the second best.
}
\label{tab:cls}
\vspace{-7mm}
\end{table}

==> tables/tab_modelnet_ablation.tex <==
\begin{table}[]
\small
\addtolength{\tabcolsep}{2pt}
\centering
\begin{tabular}{c|c|c|c}
%\hline
%Methods &  Mean pool & Max pool & Unsup. atten. & Point conv & Full    \\ \hline
%Accuracy & ? & 87.4 & ? & ? & \textbf{88.3}\\ \hline
%\end{tabular}
\hline
conv &  global pool & Loss & Acc (\%)   \\ \hline
Separable Conv & Attentive & $\mathcal{L}_{cls} + \mathcal{L}_{sa}$ & \textbf{88.3}\\ 
Separable Conv & Attentive & $\mathcal{L}_{cls}$  & 87.7\\ 
Separable Conv & Max & $\mathcal{L}_{cls}$  & 87.7\\ 
Separable Conv & Mean & $\mathcal{L}_{cls}$  &  87.4\\ 
Point Conv & Attentive & $\mathcal{L}_{cls} + \mathcal{L}_{sa}$  & 86.1\\ \hline
\end{tabular}
\caption{Results of ablation studies on ModelNet40 dataset. The \textit{conv} column denotes the configuration of convolution layers. The \textit{global pool} column denotes the type of global pooling method. Loss configuration follows notation from Sec.~\ref{sec:att}.
% $\mathcal{L}_{cls}$ and $\mathcal{L}_{sa}$ stand for classification and attention loss, respectively. When only trained using $\mathcal{L}_{cls}$, it means the attentive pooling layer is trained in an unsupervised manner.
} 
\label{tab:modelnet_abl}
\vspace{-6mm}
\end{table}
%
%\begin{table}[]
%%\small
%\addtolength{\tabcolsep}{-4pt}
%\caption{Results of ablation studies on ModelNet40 dataset. The \textit{conv} column denotes the configuration of convolution layers. The \textit{global pool} column denotes the type of global pooling method. 
%} 
%\centering
%\begin{tabular}{c|c|c|c|c}
%%\hline
%%Methods &  Mean pool & Max pool & Unsup. atten. & Point conv & Full    \\ \hline
%%Accuracy & ? & 87.4 & ? & ? & \textbf{88.3}\\ \hline
%%\end{tabular}
%Config & 1 & 2 & 3 & \\ 
% \hline
%conv & Separable & Separable & Separable & Point Conv   \\ % \hline
%pooling & Attentive & Max & Mean & Attentive\\ 
%params & 3.4M & 3.4M &  3.4M & 1.7M \\ 
%\hline
%Acc (\%) & \textbf{88.2} & 87.7 & 87.4 & 86.1\\ 
%\hline
%\end{tabular}
%
%
%\label{tab:3dm_abl}
%%\vspace{-7 pt}
%\end{table}

==> tables/tab_modelnet_pose.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\small
\centering
\addtolength{\tabcolsep}{3pt}
\begin{tabular}{c|c|c|c}
\hline
  & Mean ($^{\circ}$) & Median ($^{\circ}$) & Max($^{\circ}$) \\ \hline
 KPConv~\cite{thomas2019kpconv} & 11.46 & 8.06 & 82.32\\
 Ours-20 & 1.36 & 1.16 & 8.30\\ 
 Ours-60 & \textbf{1.25} & \textbf{1.11} & \textbf{6.63} \\ \hline
\end{tabular}
\caption{Angular errors in point cloud pose estimation. 
	%We compare our testing accuracy with previous methods on rotated ModelNet40 dataset, where each training and testing data is perturbed with a random rotation
	%color in \textcolor{blue}{blue} denotes the second best.
}
\label{tab:reg}
\vspace{-1mm}
\end{table}
